A Comprehensive Survey of Hallucination Mitigation Techniques in Large Language Models

As Large Language Models (LLMs) continue to advance in their ability to write human-like text, a key challenge remains around their tendency to hallucinate generating content that appears factual but is ungrounded. This issue of hallucination is arguably the biggest hindrance to safely deploying these powerful LLMs into real-world production systems that impact people's lives. The journey toward widespread adoption of LLMs in practical settings heavily relies on addressing and mitigating hallucinations. Unlike traditional AI systems focused on limited tasks, LLMs have been exposed to vast amounts of online text data during training. While this allows them to display impressive language fluency, it also means they are capable of extrapolating information from the biases in training data, misinterpreting ambiguous prompts, or modifying the information to align superficially with the input. This becomes hugely alarming when we rely on language generation capabilities for sensitive applications, such as summarizing medical records, financial analysis reports, etc. This paper presents a comprehensive survey of over 32 techniques developed to mitigate hallucination in LLMs. Notable among these are Retrieval Augmented Generation (Lewis et al, 2021), Knowledge Retrieval (Varshney et al,2023), CoNLI (Lei et al, 2023), and CoVe (Dhuliawala et al, 2023). Furthermore, we introduce a detailed taxonomy categorizing these methods based on various parameters, such as dataset utilization, common tasks, feedback mechanisms, and retriever types. This classification helps distinguish the diverse approaches specifically designed to tackle hallucination issues in LLMs. Additionally, we analyze the challenges and limitations inherent in these techniques, providing a solid foundation for future research in addressing hallucinations and related phenomena within the realm of LLMs.

==> table.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=40 em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                text centered,
                minimum width=5em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=15em,font=\normalsize,}{},
            where level=2{text width=14em,font=\normalsize,}{},
            where level=3{text width=30em,font=\normalsize,}{},
            where level=4{text width=22em,font=\normalsize,}{},
            where level=5{text width=18em,font=\normalsize,}{},
            [
                Hallucination Mitigation\\ Techniques in LLMs
                [
                    Prompt Engineering
                    [
                        Retrieval-based \\ Post-hoc Editing
                        [LLM-Augmenter \cite{peng2023check} \\ 
                        Knowledge Retrieval \cite{varshney2023stitch} \\
                        RARR \cite{gao2023rarr} \\
                        FreshPrompt \cite{vu2023freshllms} \\
                        High Entropy Word Spotting and Replacement \cite{rawte2023troubling} 
                            , leaf
                        ]
                    ]
                    [
                        Self Refinement through \\ Feedback and Reasoning
                        [Prompting GPT-3 To Be Reliable \cite{si2022prompting} \\
                        ChatProtect \cite{mündler2023selfcontradictory} \\
                        Self-Reflection Methodology \cite{ji2023mitigating} \\
                        Decompose-and Query framework (D\&Q) \cite{cao2023step} \\
                        Structured Comparative reasoning \cite{yan2023basis} \\
                        EVER \cite{kang2023ever} \\
                        Mind’s Mirror \cite{liu2023minds} \\
                        DRESS \cite{chen2023dress} \\
                        MixAlign \cite{zhang2023knowledge} \\
                        CoVe \cite{dhuliawala2023chainofverification} \\
                        CoNLI \cite{lei2023chain} 
                            , leaf
                        ]
                    ]
                    [
                        Prompt Tuning
                        [UPRISE \cite{cheng2023uprise} \\
                        SynTra \cite{jones2023teaching} 
                            , leaf
                        ]
                    ]
                ]

                [
                    Developing Models
                    [
                        Introducing New Decoding \\ Strategy
                        [
                            CAD \cite{shi2023trusting} \\
                            DoLa \cite{chuang2023dola} \\
                            Inference-Time Intervention (ITI) \cite{li2023inference} 
                            , leaf
                        ]
                    ]
                    [
                        Utilization of Knowledge Graph
                        [RHO \cite{ji-etal-2023-rho} \\
                            FLEEK \cite{bayat2023fleek} 
                            , leaf
                        ]
                    ]
                    [
                        Introducing Faithfulness \\ based Loss Function
                        [
                                THAM Framework \cite{yoon-etal-2022-information} \\
                                Loss Weighting Method \cite{qiu2023detecting} 
                            , leaf
                        ]
                    ]
                    [
                        Supervised Finetuning
                        [
                            Knowledge Injection and Teacher-Student Approach \cite{elaraby2023halo} \\
                            HAR \cite{köksal2023hallucination} \\
                            Fine-tuning Language Models for Factuality \cite{tian2023finetuning} \\
                            BEINFO \cite{razumovskaia2023textitdial} \\
                            R-Tuning \cite{zhang2023r} \\
                            TWEAK \cite{qiu2023think} 
                            , leaf
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy for Hallucination Mitigation Techniques in Large Language Models focusing on existing/new model development and prompting techniques. The model development has several internal fine-tuning or knowledge graph-based optimizations whereas feedback and retrievals are highlighted in the prompt engineering section}
    \label{fig:lit_surv}
\end{figure*}
